Grammar Induction from Visual, Speech and Text

Grammar Induction could benefit from rich heterogeneous signals, such as text, vision, and acoustics. In the process, features from distinct modalities essentially serve complementary roles to each other. With such intuition, this work introduces a novel \emph{unsupervised visual-audio-text grammar induction} task (named \textbf{VAT-GI}), to induce the constituent grammar trees from parallel images, text, and speech inputs. Inspired by the fact that language grammar natively exists beyond the texts, we argue that the text has not to be the predominant modality in grammar induction. Thus we further introduce a \emph{textless} setting of VAT-GI, wherein the task solely relies on visual and auditory inputs. To approach the task, we propose a visual-audio-text inside-outside recursive autoencoder (\textbf{VaTiora}) framework, which leverages rich modal-specific and complementary features for effective grammar parsing. Besides, a more challenging benchmark data is constructed to assess the generalization ability of VAT-GI system. Experiments on two benchmark datasets demonstrate that our proposed VaTiora system is more effective in incorporating the various multimodal signals, and also presents new state-of-the-art performance of VAT-GI.

==> figures/app_obj_dist.tex <==
% \pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.7)}}}
\pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.45)}, font=\fontsize{14}{1}\selectfont},every axis/.append style={xtick pos=left,ytick pos=left,tickwidth=1.5pt}}
\usetikzlibrary{matrix}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{patterns,backgrounds}

\definecolor{c1}{RGB}{252,232,212}
\definecolor{c2}{RGB}{184,183,163}
\definecolor{c3}{RGB}{107,112,092}
\definecolor{c4}{RGB}{203,153,126}
\definecolor{c5}{RGB}{107,112,092}

\begin{figure*}[t]
\centering
\begin{tikzpicture}
%\begin{groupplot}[group style={group name=myplot,group size=2 by 1,horizontal sep=30pt,xlabels at=edge bottom, ylabels at=edge left},height=4cm,width=4cm]
\begin{axis}[
	ybar,
	ytick = {0, 5, 10},
	yticklabels={0, 5, 10},
	ymax=11,ymin=0.5,
	ylabel = \%,
	y tick label style = {yshift=-0.5em, text height=0ex,font=\scriptsize},
	%    ytick style = {yshift=-0.0em, font=\scriptsize},
    x label style = {font=\scriptsize},
    y label style = {yshift=-0.5em,font=\scriptsize},
	axis line style={-},
    axis x line*=bottom,
    axis y line*=left,
	enlargelimits=0.05,
	xticklabels={man, building, tree, table, window, wall, woman, car, water, sky, fence, person, plant, grass, chair, sign, train, road, plate, street},
	xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
	xmax=20, xmin=1,
	x tick label style = {yshift=0.05em,rotate=90, align=center,font=\small},
%	title=(a) BLEU-4,
	title style={yshift=-0.9em,font=\small},
    ymajorgrids,
	width = \textwidth,
	height = 5cm,
        legend style={at={(0.67,1.04)},anchor=north west, legend columns=-1, font=\scriptsize},
	]
	\addplot[c4, pattern= north east lines, thick, pattern color=c4, bar shift=-0.25em, bar width = 0.5em] coordinates
	{
	(1,11)
        (2,7.6)
        (3,5.4)
        (4,4.4)
        (5,4.4)
        (6,3.9)
        (7,3.7)
        (8,3.4)
        (9,3.1)
        (10,3.0)
        (11,2.6)
        (12,2.5)
        (13,2.4)
        (14,2.4)
        (15,2.4)
        (16,2.4)
        (17,2.2)
        (18,2.1)
        (19,1.9)
        (20,1.8)
	};\addlegendentry{SpokenCOCO}

 \addplot[c3, pattern= north east lines, thick, pattern color=c3, bar shift=0.25em, bar width = 0.5em] coordinates
	{
	(1,6.5)
        (2,6.4)
        (3,6.2)
        (4,6.0)
        (5,6.3)
        (6,5.9)
        (7,5.7)
        (8,5.5)
        (9,5.9)
        (10,5.3)
        (11,4.9)
        (12,4.4)
        (13,4.6)
        (14,4.1)
        (15,3.7)
        (16,3.9)
        (17,3.1)
        (18,3.3)
        (19,3.5)
        (20,3.0)
	};\addlegendentry{SpokenCOCO}

    % \addplot[c2, pattern= north east lines, thick, pattern color=c2, bar shift=0pt, bar width = 1em] coordinates
	% {
	% 	(2,  26.23)
	% };
	
	% \addplot[c3, pattern=crosshatch, pattern color=c3, thick, bar shift=0pt, bar width = 1em] coordinates
	% {
	% 	(2.7,  26.40)
	% };
\end{axis}

\end{tikzpicture}
\caption{20 main types of objects distribution in SpokenCOCO and SpokenStory dataset.}
\label{fig:tag_dist}
\end{figure*}


==> figures/human_speech.tex <==
% \pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.7)}}}
\pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.45)}, font=\fontsize{14}{1}\selectfont},every axis/.append style={xtick pos=left,ytick pos=left,tickwidth=1.5pt}}
\usetikzlibrary{matrix}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{patterns,backgrounds}

\definecolor{c1}{RGB}{252,232,212}
\definecolor{c2}{RGB}{184,183,163}
\definecolor{c3}{RGB}{107,112,092}
\definecolor{c4}{RGB}{203,153,126}
\definecolor{c5}{RGB}{107,112,092}

\begin{figure}[!pt]
% \begin{minipage}{0.55\linewidth}
\centering
\begin{tikzpicture}
%\begin{groupplot}[group style={group name=myplot,group size=2 by 1,horizontal sep=30pt,xlabels at=edge bottom, ylabels at=edge left},height=4cm,width=4cm]
\begin{axis}[
	ybar,
	ytick = {61, 62, 63, 64, 65},
	yticklabels={61, 62, 63, 64, 65},
	ymax=65,ymin=61,
	ylabel = Corpus-F1,
	y tick label style = {yshift=-0.5em, text height=0ex,font=\scriptsize},
	%    ytick style = {yshift=-0.0em, font=\scriptsize},
    x label style = {font=\scriptsize},
    y label style = {yshift=-0.5em, font=\scriptsize},
    axis x line*=bottom,
	axis line style={-},
    axis y line*=left,
	axis line style={-},
	enlargelimits=0.05,
    nodes near coords,
    every node near coord/.append style={black, font=\tiny, opacity=0.7, yshift=-0.0em,xshift=0.0em },
	legend style={at={(0.02,0.99)},anchor=north west, draw=none, legend columns=-1, font=\scriptsize},
	xticklabels={Human,TTS},
	xtick={2,6},
% 	ymajorgrids,
	xmax=7.5, xmin=0.5,
	x tick label style = {yshift=0.4em, align=center,font=\small},
%	title=(a) BLEU-4,
	title style={yshift=-0.9em,font=\small},
	width = 10cm,
	height = 4.5cm,
	]
	\addplot[c4, pattern= north east lines, thick, pattern color=c4, bar shift=0pt, bar width = 1.6em] coordinates
	{
		(1.34,  62.70)
	};\addlegendentry{Corpus-F1}
	
	\addplot[c3, pattern=crosshatch, pattern color=c3, thick, bar shift=0pt, bar width = 1.6em] coordinates
	{
		(2.66,  63.00)
	};\addlegendentry{Sent-F1}
\end{axis}

\begin{axis}[
	ybar,
	ytick = {61, 62, 63, 64, 65},
	yticklabels={61, 62, 63, 64, 65},
	ymax=65,ymin=61,
	ylabel = Sent-F1,
	y tick label style = {yshift=-0.5em, text height=0ex,font=\scriptsize},
%   ytick style = {yshift=-0.0em, font=\scriptsize},
	x label style = {font=\scriptsize},
    y label style = {yshift=0.5em,font=\scriptsize},    
	axis y line*=right,
	enlargelimits=0.05,
    nodes near coords,
    every node near coord/.append style={black, font=\tiny, opacity=0.7, yshift=-0.em,xshift=0.0em },
	%legend style={at={(0,1.04)},anchor=north west, legend columns=-1, font=\scriptsize},
	xticklabels={SPICE},
	%xtick={7},
	xmax=7.5, xmin=0.5,
	% x tick label style = {xshift=-5em, yshift=0.05em, align=center,font=\small},
%	title=(a) BLEU-4,
	title style={yshift=-0.9em,font=\small},
	% width = 7cm,
	% height = 3.6cm,
	width = 10cm,
	height = 4.5cm,
	axis x line*=top,
	axis line style={-},
	xtick=\empty,
	]
	
	\addplot[c4, pattern= north east lines, thick, pattern color=c4, bar shift=0pt, bar width = 1.6em] coordinates
	{
		(5.34,  61.55)
	};
	\addplot[c3, pattern=crosshatch, pattern color=c3, thick, bar shift=0pt, bar width = 1.6em] coordinates
	{
		(6.66,  61.97)
	};
%	\addlegendentry{Pipeline}
%	\addplot[red, pattern=dots, pattern color=red, thick, bar shift=0pt, bar width = 1.6em] coordinates
%	{
%	(4.16,  32.58)
%	}
\end{axis}
\end{tikzpicture}
% \vspace{-2mm}
\caption{
Comparison of SpeechCOCO (``TTS'' ) and SpokenCOCO (``Human''). 
% ``Human'' means the results on SpokenCOCO while ``TTS'' means the results on SpeechCOCO.
}
\label{fig:human_speech}
\vspace{-3mm}
% \end{minipage}
% \quad
% \begin{minipage}{0.40\linewidth}
    % \begin{table}
        % \fontsize{8}{10}\selectfont
        % \setlength{\tabcolsep}{2.mm}
        % \begin{center}
        % % \resizebox{1\textwidth}{!}{
        % \vspace{-4mm}
        % \captionof{table}{\small
        % Corpus-F1 of VaTiora on the SpokenCOCO with different SNR. Smaller SNR means heavier noise.
        % }
        % % \vspace{2mm}
        % \begin{tabular}{ccc}
        % \hline
        % \bf SNR (dB) & \bf Corpus-F1 (\%)\\
        % \hline
        % -5 & 55.31 \\
        % 0 & 58.24 \\
        % 5 &  61.92 \\
        % 10 & 62.04 \\

        % \hline
        % \end{tabular}
        % % }
        % \label{tab:noise}
        % \end{center}
        % \vspace{-5mm}
    % \end{table}
% \end{minipage}
\end{figure}



==> figures/length.tex <==
% \pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.7)}}}
% \pgfplotsset{compat=1.7,every axis title/.append style={at={(0.5,-0.45)}, font=\fontsize{14}{1}\selectfont},every axis/.append style={xtick pos=left,ytick pos=left,tickwidth=1.5pt}}
\usetikzlibrary{matrix}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{patterns,backgrounds}

\definecolor{c0}{RGB}{255,0,0}
\definecolor{c1}{RGB}{0,0,255}
\definecolor{c2}{RGB}{184,183,163}
\definecolor{c3}{RGB}{107,112,092}
\definecolor{c4}{RGB}{203,153,126}
\definecolor{c5}{RGB}{107,112,092}

\begin{figure*}[t]
\centering
\begin{tikzpicture}
\pgfplotsset{set layers=standard}
\begin{groupplot}[group style={group name=myplot,group size=2 by 1,horizontal sep=30pt,xlabels at=edge bottom, ylabels at=edge left},height=9cm,width=8.5cm]
% \begin{axis}
    \nextgroupplot
    [
	% yline,
    smooth,
	ytick = {0, 20, 40, 60, 80, 100},
	% yticklabels={20, 40, 60, 80, 100},
	ymax=100,ymin=0,
	ylabel = {Recal (\%)},
    y label style = {yshift=-0.9em,xshift=0em,font=\scriptsize,align=center},
	y tick label style = {yshift=-0.5em,xshift=0.1em, text height=0ex,font=\scriptsize},
%   ytick style = {yshift=-0.0em, font=\scriptsize},
    xtick= {2,4,6,8,10,12,14,16,18,20,22,24,26,28,30},
% 	ymajorgrids,
	xmax=18, xmin=1,
    ymajorgrids,
    grid style=dashed,
	x tick label style = { align=center,font=\scriptsize},
	title=(a) SpokenCOCO,
	title style={yshift=0,font=\small},
    width = 0.6\textwidth,
	height = 4.0cm,
    legend style={at={(0.2,1.25)},anchor=north west, legend columns=-1, font=\scriptsize},
    ]
    \addplot+[
        mark=square*,
        opacity=0.5,
        mark options={c0,scale=0.5pt},
        c0
    ] coordinates
    {
        (2,  90.01)
        (3,  87.63)
        (4,  77.18)
        (5,  71.09)
        (6,  65.26)
        (7,  61.71)
        (8,  62.80)
        (9,  62.38)
        (10, 61.62)
        (11, 57.28)
        (12, 58.11)
        (13, 55.94)
        (14, 54.20)
        (15, 55.03)
        (16, 55.73)
        (17, 53.22)
    };\addlegendentry{VaTiora}

	\addplot+[
        mark=*,
        mark options={c4,scale=0.5pt},
        c4
    ] coordinates
	{
        (2,  82.28)
        (3,  74.63)
        (4,  63.18)
        (5,  61.09)
        (6,  60.26)
        (7,  59.71)
        (8,  57.80)
        (9,  56.38)
        (10, 50.62)
        (11, 49.28)
        (12, 51.11)
        (13, 52.94)
        (14, 52.20)
        (15, 49.03)
        (16, 43.73)
        (17, 41.22)
	};\addlegendentry{Cliora}
%	\addplot[red, pattern=dots, pattern color=red, thick, bar shift=0pt, bar width = 1.6em] coordinates
%	{
%	(4.16,  32.58)
%	}
% \end{axis}
    \addplot+[
        mark=x,
        mark options={c2,scale=0.5pt},
        c2
    ] coordinates
	{
        (2,  80.01)
        (3,  70.63)
        (4,  61.18)
        (5,  60.09)
        (6,  57.26)
        (7,  58.71)
        (8,  55.80)
        (9,  56.38)
        (10, 50.62)
        (11, 49.28)
        (12, 47.17)
        (13, 43.94)
        (14, 41.20)
        (15, 40.21)
        (16, 39.73)
        (17, 40.22)
	};\addlegendentry{Diora}

    \addplot+[
            mark=triangle*,
            opacity=0.5,
            mark options={c1,scale=1pt},
            c1
    ] coordinates
	{
        (2,  60.01)
        (3,  70.63)
        (4,  64.18)
        (5,  60.09)
        (6,  59.26)
        (7,  57.71)
        (8,  58.80)
        (9,  56.38)
        (10, 59.62)
        (11, 56.28)
        (12, 55.11)
        (13, 54.94)
        (14, 55.20)
        (15, 51.13)
        (16, 48.73)
        (17, 47.22)
	};\addlegendentry{VC-PCFG}

    \addplot+[
            mark=diamond*,
            mark options={c5,scale=1pt},
            c5
    ] coordinates
	{
        (2,  50.01)
        (3,  55.63)
        (4,  57.18)
        (5,  53.09)
        (6,  48.26)
        (7,  43.71)
        (8,  42.80)
        (9,  44.38)
        (10, 43.62)
        (11, 44.28)
        (12, 47.11)
        (13, 45.94)
        (14, 42.20)
        (15, 41.10)
        (16, 42.69)
        (17, 40.22)
	};\addlegendentry{C-PCFG}

    \addplot[
        mark=o,
        mark options={c5,scale=1pt},
        c5
    ] coordinates
    {
        (2,  71.01)
        (3,  67.63)
        (4,  55.18)
        (5,  44.09)
        (6,  37.26)
        (7,  28.71)
        (8,  26.80)
        (9,  25.38)
        (10, 18.62)
        (11, 17.28)
        (12, 16.11)
        (13, 14.94)
        (14, 9.20)
        (15, 7.03)
        (16, 17.73)
        (17, 23.25)
    };\addlegendentry{VG-NSL}

    \nextgroupplot
    [
	% yline,
    smooth,
	ytick = {0, 10, 20, 30, 40, 50, 60},
	% yticklabels={20, 40, 60, 80, 100},
	ymax=60,ymin=0,
	% ylabel = {Recal (\%)},
    y label style = {yshift=-0.5em,xshift=0em,font=\scriptsize,align=center},
	y tick label style = {yshift=-0.5em,xshift=0.1em, text height=0ex,font=\scriptsize},
%   ytick style = {yshift=-0.0em, font=\scriptsize},
    xtick= {2,4,6,8,10,12,14,16,18,20,22,24,26,28,30},
% 	ymajorgrids,
	xmax=31, xmin=19,
    ymajorgrids,
    grid style=dashed,
	x tick label style = { align=center,font=\scriptsize},
	title=(b) SpokenStory,
	title style={yshift=0,font=\small},
    width =0.45\textwidth,
	height = 4.0cm,
    legend style={at={(0.98,1.30)},anchor=north west, legend columns=-1, font=\scriptsize},
    ]
    \addplot+[
        mark=square*,
        opacity=0.5,
        mark options={c0,scale=0.5pt},
        c0
    ] coordinates
    {
        (20,  57.03)
        (21,  56.11)
        (22,  54.21)
        (23,  53.32)
        (24,  53.18)
        (25,  52.09)
        (26,  50.26)
        (27,  49.71)
        (28,  48.80)
        (29,  45.38)
        (30,  41.62)
    };

    \addplot+[
        mark=*,
        mark options={c4,scale=0.5pt},
        c4
    ] coordinates
	{
        (20,  44.09)
        (21,  40.17)
        (22,  39.52)
        (23,  37.63)
        (24,  36.18)
        (25,  34.09)
        (26,  31.26)
        (27,  32.71)
        (28,  26.72)
        (29,  24.38)
        (30,  25.62)
	};

    \addplot+[
        mark=x,
        mark options={c2,scale=0.5pt},
        c2
    ] coordinates
	{
        (20,  45.11)
        (21,  37.31)
        (22,  34.09)
        (23,  31.63)
        (24,  28.18)
        (25,  26.09)
        (26,  27.23)
        (27,  21.67)
        (28,  19.82)
        (29,  24.40)
        (30,  22.59)
	};


\end{groupplot}
\end{tikzpicture}
% \vspace{-3mm}
\caption{
Recall curves varying by constituent length on SpokenCOCO and SpokenStory. 
% For a span $(i,j)$, constituent length is $j-i$.
}
\label{fig:constituent length}
% \vspace{-2mm}
\end{figure*}


==> tables/app_obj.tex <==
\begin{wraptable}{r}{0.57\linewidth}
    \vspace{-10mm}
    \fontsize{9}{11.5}\selectfont
    \setlength{\tabcolsep}{2mm}
    
    \begin{center}
    % \resizebox{1\textwidth}{!}{
    % \vspace{-8mm}
    \caption{\small
    Corpus-F1 results of different RoI numbers in each image on SpokenCOCO test set.
    }
    % \vspace{-2mm}
    \begin{tabular}{cccccccc}
    \hline
     RoI NUM & \bf Corpus-F1\\
    \hline
     3 & 58.01 \\
     10 & 60.10 \\
     36 & \bf 62.70 \\
     100 & 62.58 \\

    \hline
    \end{tabular}
    % }
    \label{tab:obj}
    \end{center}
    \vspace{-3mm}
\end{wraptable}

==> tables/group_table.tex <==
\begin{table}[t]
\begin{minipage}[t]{0.45\linewidth}
    \fontsize{8}{10}\selectfont
    \setlength{\tabcolsep}{1.mm}    
    \begin{center}
    % \resizebox{1\textwidth}{!}{
    % \vspace{-10mm}
    \caption{\small
    Main results on the SpokenCOCO using Corpus-F1 and Sent-F1. In the VAT-GI-Textless setting, we report Corpus-SCF1 and Sent-SCF1.
    }
    \vspace{0.5mm}
    \begin{tabular}{lccc}
    \hline
    \multicolumn{1}{c}{} & \bf Corpus-F1 & \bf Sent-F1\\
    \hline
    \multicolumn{3}{l}{$\bullet$ \textbf{Text-only GI}} \\
    \quad Left Branch & 15.1 & 15.7\\
    \quad Right Branch & 51.0 & 51.8\\
    \quad Random & 24.2 & 24.6\\
    \quad C-PCFG & 53.6 & 53.7\\
    \quad Diora & 58.3 & 59.1 \\
    \cdashline{1-4}
    % Vision-language 
    \multicolumn{3}{l}{$\bullet$ \textbf{Visual-Text GI}} \\
    \quad VG-NSL & 50.4 & -\\
    \quad VG-NSL+HI & 53.3 & -\\
    \quad VC-PCFG & 59.3 & 59.4\\
    \quad Cliora & 61.0 & 61.7\\
    \cdashline{1-4}
    \multicolumn{3}{l}{$\bullet$ \textbf{VAT-GI}} \\
    \quad VaTiora & \bf 62.7 & \bf 63.0\\
    \hline
    \multicolumn{1}{c}{} & \bf Corpus-SCF1 & \bf Sent-SCF1\\
    \cdashline{1-4}
    \multicolumn{3}{l}{$\bullet$ \textbf{VAT-GI-Textless}} \\
    % \quad VaTiora (Textless) & 32.45 & 31.19\\    
    \quad VaTiora & 32.5 & 31.2\\

    \hline
    \end{tabular}
    % }
    \label{tab:main_results}
    \end{center}
    % \vspace{-5mm}
\end{minipage}
% \medskip
\quad
\begin{minipage}[t]{0.50\linewidth}
\fontsize{8}{10}\selectfont
    \setlength{\tabcolsep}{0.5mm}
    
    \begin{center}
    % \resizebox{1\textwidth}{!}{
    % \vspace{-6.5mm}
    \caption{\small
    Statistics of SpokenCOCO and SpokenStory. 
    We follow \cite{DBLP:journals/pami/KarpathyF17} to split SpokenCOCO. ``Avg.Speech Len.'' and ``Avg.Sent.Len.'' means the average speech and sentence length, respectively. 
    % ``$\star$'' means the number is for the whole OpenImage images.
    % SpokenStory dataset and SpokenCOCO test set.
    }
    \vspace{0.5mm}
    \begin{tabular}{lccc}
    \hline
    \multicolumn{1}{c}{} & \small{\bf SpokenCOCO} & \small{\bf SpokenStory} \\
    \hline
    Split & Train/Val/Test & Test \\
    % \hline
    % \multicolumn{4}{l}{\textbf{2D vs. 3D Info}} \\
    % & 2D & - & - \\
    % & 3D & - & - \\
    Images & 80K/5K/5K & 1K \\
    Visual scenario & 91 & > 300 \\
    \cdashline{1-3}
    Avg. Speech Len. (sec.) & 2.54 & 5.01 \\
    Tone Styles & Monotonous & 5 Styles \\
    \cdashline{1-3}
    Avg. Sent. Len. (word) & 10.46 & 20.69 \\
    \hline
    \end{tabular}
    % }
    \label{tab:data}
    \end{center}
    % \vspace{-3mm}
    \fontsize{9}{11}\selectfont
    \setlength{\tabcolsep}{2mm}
    \begin{center}
    % \resizebox{1\textwidth}{!}{
    % \vspace{1.6mm}
    \caption{\small
    Corpus-F1 on the SpokenCOCO test set and SpokenStory. 
    All models are trained on the SpokenCOCO train set.
    }
    \vspace{-5mm}
    \begin{tabular}{lccc}
    \hline
    \multicolumn{1}{c}{} & \bf SpokenCOCO & \bf SpokenStory\\
    \hline
    $\bullet$ \textbf{Avg.Sent.Len.} & 10.46 & 20.69 \\
    \hline
    \quad Diora & 58.30 & 35.74 \\
    \quad Cliora & 61.00 & 37.82 \\
    \quad VaTiora & \bf 62.70 & \bf 53.19 \\
    \hline
    \end{tabular}
    % }
    \label{tab:res_story}
    \end{center}
    % \vspace{-4mm}
\end{minipage}
\vspace{-4mm}
\end{table}

==> tables/label.tex <==
\definecolor{c1}{RGB}{252,232,212}
\definecolor{c2}{RGB}{184,183,163}
\definecolor{c3}{RGB}{107,112,092}
\definecolor{c4}{RGB}{203,153,126}
\definecolor{c5}{RGB}{107,112,092}

\begin{figure*}[!t]
    \centering
    \begin{tikzpicture}
    \pgfplotsset{set layers=standard}
    % \begin{groupplot}[group style={group name=myplot,group size=2 by 1,horizontal sep=30pt,xlabels at=edge bottom, ylabels at=edge left},height=9cm,width=8.5cm]
    % \begin{semilogyaxis}
    \begin{axis}
        [
        % yline,
        ybar,
        yshift=-0.84cm,
        xshift=-0.36cm,
        ytick = {0, 30, 50},
        yticklabels={0, 25, 50},
        ymax=55,ymin=0,
        log origin=infty,
        ylabel = {Proportion(\%)},
        y label style = {rotate=-90,yshift=0.0em,xshift=1.8em,font=\scriptsize,rotate=90, align=center},
        y tick label style = {yshift=-0.5em,xshift=0.1em, text height=0ex,font=\scriptsize},
    %   ytick style = {yshift=-0.0em, font=\scriptsize},
        xtick= \empty,
    % 	ymajorgrids,
        xmax=100, xmin=0,
        ymajorgrids,
        grid style=dashed,
        % x tick label style = {xshift=-5em, yshift=0.05em, align=center,font=\small},
    %	title=(a) BLEU-4,
        title style={yshift=-0.9em,font=\small},
        width = 14.8cm,
        height = 4.5cm,
        ]
        \addplot+[
            mark=*,
            mark options={c4,scale=0.5pt},
            c4,thick
        ] coordinates
        {
            (21,  51.14)
            (32,  15.50)
            (42.3,  22.26)
            (52.3,  7.37)
            (63,  1.14)
            (74,  1.15)
            (84,  0.01)
            (94.5,  0.01)
        };
    % \end{semilogyaxis}
    \end{axis}
    \end{tikzpicture}
% \begin{table}[t]
    % \setlength{\tabcolsep}{6pt}
    \fontsize{9.5}{11}\selectfont
    % \fontsize{8}{10.5}\selectfont
    \setlength{\tabcolsep}{2.8mm}
    % \vspace{-2mm}
    \begin{center}
    % \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{clccccccccccccc}
    \hline
    & \bf NP & \bf VP & \bf PP & \bf S & \bf SBAR & \bf ADJP & \bf QP & \bf ADVP\\
    \hline
    Left Branch & 33.20 & 0.00 & 0.10 & 0.00 & 0.00 & 4.90 & 0.00 & 0.00 \\
    Right Branch & 37.50 & \bf 94.50 & 71.10 & 0.00 & \bf 97.80 & 20.90 & 0.00 & 79.10 \\
    Random & 32.80 & 18.40 & 24.40 & 0.10 & 17.70 & 26.80 & 0.00 & 20.90 \\
    C-PCFG$^\dag$ & 43.00 & 85.00 & 78.40 & - & 90.60 & 36.60 & - & \bf 87.40 \\
    Diora$^\star$ & 68.20 & 55.89 & 52.96 & 71.02 & 54.56 & 53.76 & 71.29 & 61.68\\
    \hline
    VG-NSL$^\dag$ & 64.30 & 28.10 & 32.20 & - & 16.90 & 13.20 & - & 5.60\\
    VG-NSL+HI$^\dag$ & 61.00 & 33.50 & 62.70 & - & 42.00 & 13.90 & - & 65.90 \\
    VC-PCFG$^\dag$ & 54.90 & 83.20 & \bf 80.90 & - & 89.00 & 38.80 & - & 86.30 \\
    Cliora$^\star$ & 70.38 & 56.82 & 51.70 & 73.34 & 57.01 &  56.91 & 68.74 & 66.48\\
    \hline
    VaTiora & \bf 71.92 & 60.17 & 53.05 & \bf 74.58 & 59.40 & \bf 58.22 & \bf 71.35 & 65.10 \\
    w/o Vision & 67.04 &	58.82 &	50.97 &	75.11 &	59.40 &	58.21 &	71.35 &	65.30\\
    w/o Speech & 70.40 & 55.95 & 52.97 & 73.40 & 59.40 &	58.01 &	71.66 &	65.10\\
    \hline
    \end{tabular}
    % }
    \end{center}
    % \vspace{-1mm}
    \caption{
        Recall of eight constituent labels on SpokenCOCO test set. The best mean number in each column is in bold. \dag\ indicates results reported by \citet{DBLP:conf/emnlp/ZhaoT20}. $\star$ indicates the results are obtained by running their code on our dataset. The bar chart describes the distribution of each label.
    }
    \label{fig:label}
% \end{table}
    % \vspace{-5mm}
\end{figure*}
